Using Gaussian Measures for Efficient Constraint Based Clustering

In this paper we present a novel iterative multiphase clustering technique for efficiently clustering high dimensional data points. For this purpose we implement clustering feature (CF) tree on a real data set and a Gaussian density distribution constraint on the resultant CF tree. The post processing by the application of Gaussian density distribution function on the micro-clusters leads to refinement of the previously formed clusters thus improving their quality. This algorithm also succeeds in overcoming the inherent drawbacks of conventional hierarchical methods of clustering like inability to undo the change made to the dendogram of the data points. Moreover, the constraint measure applied in the algorithm makes this clustering technique suitable for need driven data analysis. We provide veracity of our claim by evaluating our algorithm with other similar clustering algorithms. Introduction

==> FIXES39 <==
Version 3.9 fixes lots of bugs and this list is selective.

* \select@language did not set \languagename. This meant the language
  in force when auxiliary files were loaded was the one used in, for
  example, shorthands -- if the language was german, a
  \select@language{spanish} had no effect.

* \foreignlanguage and otherlanguage* messed up
   \extras<language>. Scripts, encodings and many other things were
   not switched correctly.

* The :ENC mechanism for hyphenation patterns used the encoding of the
  _previous_ language, not that of the language being selected.

* ' (with activeacute) had the original value when writing to an
  auxiliary file, and things like an infinite loop could happen. It
  worked incorrectly with ^ (if activated) and also if deactivated.

* Active chars where not reset at the end of language options, and
  that lead to incompatibilities between languages.

* \textormath raised and error with a conditional.

* \aliasshorthand didn't work (or only in a few and very specific
  cases).

* \l@english was defined incorrectly (using \let instead of \chardef).

* ldf files not bundled with babel were not recognized when called as global
  options.
 


==> Gaussian Clustering/FIXES39 <==
Version 3.9 fixes lots of bugs and this list is selective.

* \select@language did not set \languagename. This meant the language
  in force when auxiliary files were loaded was the one used in, for
  example, shorthands -- if the language was german, a
  \select@language{spanish} had no effect.

* \foreignlanguage and otherlanguage* messed up
   \extras<language>. Scripts, encodings and many other things were
   not switched correctly.

* The :ENC mechanism for hyphenation patterns used the encoding of the
  _previous_ language, not that of the language being selected.

* ' (with activeacute) had the original value when writing to an
  auxiliary file, and things like an infinite loop could happen. It
  worked incorrectly with ^ (if activated) and also if deactivated.

* Active chars where not reset at the end of language options, and
  that lead to incompatibilities between languages.

* \textormath raised and error with a conditional.

* \aliasshorthand didn't work (or only in a few and very specific
  cases).

* \l@english was defined incorrectly (using \let instead of \chardef).

* ldf files not bundled with babel were not recognized when called as global
  options.
 


==> Gaussian Clustering/README <==
Babel 3.9l
----------

This is Babel 3.9l.

Version 3.9a fixed lots of bugs and added some new features, intended
mainly to make it compatible somehow with Unicode engines. Some bugs
have not been fixed to avoid backward incompatibilities, but they have
been documented. Most of the new features (like package options) are
intended to overcome issues in previous releases without changing
significantly the behaviour of Babel.

Languages are not part of the Babel core any more; in particular, it
shall be no longer necessary to synchronize Babel core releases with
releases of Babel language files. See CONTRIB for further details
about contributing a language.

To install it, just tex babel.ins and move the generated files to the
corresponding place in your TeX distribution. Unlike former releases,
formats must not be recreated, but it is recommended, at least the
first time Babel is updated from 3.8 (or previous versions). 

Changes are described in babel.pdf with the label "New 3.9". The
manual has been expanded to include tips and tricks, but it will be
improved in next releases.

Please, report bugs and suggestions to:

http://latex-project.org/bugs-upload.html

You may also report them to the author more informally on:

http://www.tex-tipografia.com/contact.html

Bugs related to specific languages are best reported to their
respective authors.

Versions >=3.9i presumes the german style has been updated to 2.7.

New
---
* babel.dtx
3.9b  - Fixed an idiot slip in hyphen.cfg: a \def instead of \let
3.9c  - Added the "modifiers" mechanism
      - Option shorthands accepts t for ~ and c for ,
      - \foreinglanguage inserted a par (because of an empty line
        in the doc part)
3.9d  - Fixed undefined \@expandtwoargs in Plain
      - Code reorganized (just an "internal" change)
3.9e  - Fixed a bug introduced in 3.9c which mangled key=value
        options.
3.9f  - Default hyphenmins were not set to 2 3. Now they are again.
3.9g  - bbplain.dtx and babel.dtx merged.
      - The number of languages was not printed in some formats.
      - A new mechanism to force \StartBabelCommands even without the
        'strings' key (\UseStrings didn't work at all).
      - With \AfterBabelCommands macros can be defined in the global scope.
      - A tool for readjusting lccodes for hyphenation (\SetHyphenMap and a
        package option).
      - Tentative macros for \fontspec.
3.9h  - Fixed bugs in \SetStringLoop (first token expanded prematurely)
        and \SetCase (sometimes ignored).
      - bplain didn't work (again). Fixed.
      - Other minor internal changes.
3.9i  - With LuaTeX, spaces are not ignored after shorthands and closing
        braces can follow them.
      - \textlatin and friends are deprecated. For the logos (see
	below) a new macro is used if necessary (\ensureascii), so
	\textlatin is not used in the core any more.
      - \babelensure can be used to wrap caption texts with \foreignlanguage,
        as well as to enforce an encoding.
      - \babeltags is just for syntactical sugar, and defines macros
	with short names to switch the language (eg, \textdeu and \deu).
      - Partial compatibility with languages named as \lang@ instead
	of \l@ (plain etex/xetex/luatex).
      - Bug fix. The logos \TeX and \LaTeX were typeset in a wrong font
	in some cases. Now if a non-ASCII font is not loaded they are not
	redefined at all.
      - Bug fix. \bbl@allowhyphens is now ignored in vertical mode.
      - Bug fix. Loops with \@for failed in Plain.
      - Bug fix. A few codes in xetex where wrong when loading patterns.
      - Bug fix. With strings=encoded captions were left unchanged in
	\MakeUppercase/\MakeLowercase.
3.9j  - Bug fix. Plain formats didn't work (Undefined \@filelist).
3.9k  - Code and doc reorganized with some `literate' concepts (with a
        slightly patched docstrip).
      - Removed the luatex stuff for shorthands. It was just a first step,
        but ended up in the final release of 3.9i (it shouldn't).
      - Improvements for Plain and other non-LaTeX formats.
3.9l  - Formerly, fontspec set \latinencoding to EUx i babel was loaded.
        Now, babel sets it if fontspec is loaded.
      - New package options 'nocase' (\SetCase is ignored) and 'silent'
      - Improved compatibility (hopefully) with babelbib.

* bbunicode.dtx
1.0b  - Improvements by Elie Roux for LuaTeX.
1.0c  - Bug fix. A few codes in xetex where wrong when loading patterns.
   
------------
Javier Bezos
2014-09-25



==> README <==
Babel 3.9l
----------

This is Babel 3.9l.

Version 3.9a fixed lots of bugs and added some new features, intended
mainly to make it compatible somehow with Unicode engines. Some bugs
have not been fixed to avoid backward incompatibilities, but they have
been documented. Most of the new features (like package options) are
intended to overcome issues in previous releases without changing
significantly the behaviour of Babel.

Languages are not part of the Babel core any more; in particular, it
shall be no longer necessary to synchronize Babel core releases with
releases of Babel language files. See CONTRIB for further details
about contributing a language.

To install it, just tex babel.ins and move the generated files to the
corresponding place in your TeX distribution. Unlike former releases,
formats must not be recreated, but it is recommended, at least the
first time Babel is updated from 3.8 (or previous versions). 

Changes are described in babel.pdf with the label "New 3.9". The
manual has been expanded to include tips and tricks, but it will be
improved in next releases.

Please, report bugs and suggestions to:

http://latex-project.org/bugs-upload.html

You may also report them to the author more informally on:

http://www.tex-tipografia.com/contact.html

Bugs related to specific languages are best reported to their
respective authors.

Versions >=3.9i presumes the german style has been updated to 2.7.

New
---
* babel.dtx
3.9b  - Fixed an idiot slip in hyphen.cfg: a \def instead of \let
3.9c  - Added the "modifiers" mechanism
      - Option shorthands accepts t for ~ and c for ,
      - \foreinglanguage inserted a par (because of an empty line
        in the doc part)
3.9d  - Fixed undefined \@expandtwoargs in Plain
      - Code reorganized (just an "internal" change)
3.9e  - Fixed a bug introduced in 3.9c which mangled key=value
        options.
3.9f  - Default hyphenmins were not set to 2 3. Now they are again.
3.9g  - bbplain.dtx and babel.dtx merged.
      - The number of languages was not printed in some formats.
      - A new mechanism to force \StartBabelCommands even without the
        'strings' key (\UseStrings didn't work at all).
      - With \AfterBabelCommands macros can be defined in the global scope.
      - A tool for readjusting lccodes for hyphenation (\SetHyphenMap and a
        package option).
      - Tentative macros for \fontspec.
3.9h  - Fixed bugs in \SetStringLoop (first token expanded prematurely)
        and \SetCase (sometimes ignored).
      - bplain didn't work (again). Fixed.
      - Other minor internal changes.
3.9i  - With LuaTeX, spaces are not ignored after shorthands and closing
        braces can follow them.
      - \textlatin and friends are deprecated. For the logos (see
	below) a new macro is used if necessary (\ensureascii), so
	\textlatin is not used in the core any more.
      - \babelensure can be used to wrap caption texts with \foreignlanguage,
        as well as to enforce an encoding.
      - \babeltags is just for syntactical sugar, and defines macros
	with short names to switch the language (eg, \textdeu and \deu).
      - Partial compatibility with languages named as \lang@ instead
	of \l@ (plain etex/xetex/luatex).
      - Bug fix. The logos \TeX and \LaTeX were typeset in a wrong font
	in some cases. Now if a non-ASCII font is not loaded they are not
	redefined at all.
      - Bug fix. \bbl@allowhyphens is now ignored in vertical mode.
      - Bug fix. Loops with \@for failed in Plain.
      - Bug fix. A few codes in xetex where wrong when loading patterns.
      - Bug fix. With strings=encoded captions were left unchanged in
	\MakeUppercase/\MakeLowercase.
3.9j  - Bug fix. Plain formats didn't work (Undefined \@filelist).
3.9k  - Code and doc reorganized with some `literate' concepts (with a
        slightly patched docstrip).
      - Removed the luatex stuff for shorthands. It was just a first step,
        but ended up in the final release of 3.9i (it shouldn't).
      - Improvements for Plain and other non-LaTeX formats.
3.9l  - Formerly, fontspec set \latinencoding to EUx i babel was loaded.
        Now, babel sets it if fontspec is loaded.
      - New package options 'nocase' (\SetCase is ignored) and 'silent'
      - Improved compatibility (hopefully) with babelbib.

* bbunicode.dtx
1.0b  - Improvements by Elie Roux for LuaTeX.
1.0c  - Bug fix. A few codes in xetex where wrong when loading patterns.
   
------------
Javier Bezos
2014-09-25


